The dust SED of dwarf galaxies I. The case of NGC 4214

The goal of the present study is to establish the physical origin of dust heating and emission based on radiation transfer models, which self-consistently connect the emission components from diffuse dust and the dust in massive star forming regions. NGC 4214 is a nearby dwarf galaxy with a large set of ancillary data, ranging from the ultraviolet (UV) to radio, including maps from SPITZER, HERSCHEL and detections from PLANCK. We mapped this galaxy with MAMBO at 1.2 mm at the IRAM 30 m telescope. We extract separate dust emission components for the HII regions (plus their associated PDRs on pc scales) and for the diffuse dust (on kpc scales). We analyse the full UV to FIR/submm SED of the galaxy using a radiation transfer model which self-consistently treats the dust emission from diffuse and SF complexes components, considering the illumination of diffuse dust both by the distributed stellar populations, and by escaping light from the HII regions. While maintaining consistency with the framework of this model we additionally use a model that provides a detailed description of the dust emission from the HII regions and their surrounding PDRs on pc scales. Due to the large amount of available data and previous studies for NGC 4214 very few free parameters remained in the model fitting process. We achieve a satisfactory fit for the emission from HII+PDR regions on pc scales, with the exception of the emission at 8\mi, which is underpredicted by the model. For the diffuse emission we achieve a good fit if we assume that about 30-70% of the emission escaping the HII+PDR regions is able to leave the galaxy without passing through a diffuse ISM, which is not an unlikely scenario for a dwarf galaxy which has recently undergone a nuclear starburst. We determine a dust-to-gas mass ratio of 350-390 which is close to the expected value based on the metallicity.

==> Tables/STARS_NW_phot2tex.tex <==

%Table generated with dwarfSED.pro on Mon Jul 30 19:33:36 2012

%\begin{table*}
\centering
\begin{tabular}{c c c} \hline \noalign{\medskip}
\textbf{BAND} & $\lambda_{0}$($\mu$m) & $F_{\rm NW}$ (Jy) \\ \noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FUV & 0.154 & 0.017 $\pm$ 0.002 \vspace{0.15cm} \\ 
NUV & 0.232 & 0.021 $\pm$ 0.003 \vspace{0.15cm} \\ 
F225W & 0.236 & 0.022 $\pm$ 0.003 \vspace{0.15cm} \\ 
F336W & 0.335 & 0.026 $\pm$ 0.003 \vspace{0.15cm} \\ 
F438W & 0.432 & 0.038 $\pm$ 0.005 \vspace{0.15cm} \\ 
F547M & 0.545 & 0.043 $\pm$ 0.005 \vspace{0.15cm} \\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}
%\label{StarsNW}
%\caption{Region NW photometric points.}
%\end{table*}


==> Tables/STARS_SE_phot2tex.tex <==

%Table generated with dwarfSED.pro on Mon Jul 30 19:33:36 2012

%\begin{table*}
\centering
\begin{tabular}{c c c} \hline \noalign{\medskip}
\textbf{BAND} & $\lambda_{0}$($\mu$m) & $F_{\rm SE}$ (Jy) \\ \noalign{\smallskip} \hline \noalign{\medskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FUV & 0.154 & 0.007 $\pm$ 0.001 \vspace{0.15cm} \\ 
NUV & 0.232 & 0.008 $\pm$ 0.001 \vspace{0.15cm} \\ 
F225W & 0.236 & 0.007 $\pm$ 0.001 \vspace{0.15cm} \\ 
F336W & 0.335 & 0.009 $\pm$ 0.001 \vspace{0.15cm} \\ 
F438W & 0.432 & 0.013 $\pm$ 0.002 \vspace{0.15cm} \\ 
F547M & 0.545 & 0.014 $\pm$ 0.002 \vspace{0.15cm} \\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \\
\end{tabular}
%\label{StarsSE}
%\caption{Region SE photometric points.}
%\end{table*}

